Variational Inference with Gaussian Score Matching

Variational inference (VI) is a method to approximate the computationally intractable posterior distributions that arise in Bayesian statistics. Typically, VI fits a simple parametric distribution to the target posterior by minimizing an appropriate objective such as the evidence lower bound (ELBO). In this work, we present a new approach to VI based on the principle of score matching, that if two distributions are equal then their score functions (i.e., gradients of the log density) are equal at every point on their support. With this, we develop score matching VI, an iterative algorithm that seeks to match the scores between the variational approximation and the exact posterior. At each iteration, score matching VI solves an inner optimization, one that minimally adjusts the current variational estimate to match the scores at a newly sampled value of the latent variables. We show that when the variational family is a Gaussian, this inner optimization enjoys a closed form solution, which we call Gaussian score matching VI (GSM-VI). GSM-VI is also a ``black box'' variational algorithm in that it only requires a differentiable joint distribution, and as such it can be applied to a wide class of models. We compare GSM-VI to black box variational inference (BBVI), which has similar requirements but instead optimizes the ELBO. We study how GSM-VI behaves as a function of the problem dimensionality, the condition number of the target covariance matrix (when the target is Gaussian), and the degree of mismatch between the approximating and exact posterior distribution. We also study GSM-VI on a collection of real-world Bayesian inference problems from the posteriorDB database of datasets and models. In all of our studies we find that GSM-VI is faster than BBVI, but without sacrificing accuracy. It requires 10-100x fewer gradient evaluations to obtain a comparable quality of approximation.

==> gsm-alg.tex <==
\SetKwInOut{KwIn}{Input}
\SetKwInOut{KwOut}{Output}

\KwIn{Initial mean estimate $\vec{\mu_0}$,
Initial covariance estimate $\vec{\Sigma_0}$,
target distribution $p(\vec{\theta}| \vx)$, number of iterations N, batch size B}
\SetKwComment{Comment}{$\triangleright$\ }{}

\KwOut{Multivariate normal variational distribution $q_{\bw}(\vec{\theta}):=\mathcal{N}(\vec{\mu}, \vec{\Sigma}$)}

$i \leftarrow 0$ \;
\While{$i < N$}{
    $j \leftarrow 0$ \;
    \While{$j \leq B$}{
        Sample $\vec{\theta}^{(j)}\sim \mathcal{N}(\vec{\mu_{i}}, \vec{\Sigma_{i}})$ \;

        $\vec{v} \leftarrow \nabla_{\bw} \log p(\vec{\theta}^{(j)} | \vx)$ \;

        $\vec{\varepsilon}\ \leftarrow \ \mat{\Sigma}_i\vec{v} - \vec{\mu}_i + \vec{\theta}$ \;

        Solve $\rho(1\!+\!\rho)\ =\ \vec{v}^\top\mat{\Sigma}_i\vec{v} + \big[(\vec{\mu}_i\!-\!\vec{\theta})^\top\!\vec{v}\big]^2$ for $\rho>0$ \;

        $ \vec{\delta\mu}^{(j)} \leftarrow \frac{1}{1+\rho}\left[ \mI - \frac{(\vec{\mu}_i-\vec{\theta}) \vec{v}^\top}{1+\rho+ (\vec{\mu}_i-\vec{\theta})^\top \vec{v}}\right] \vec{\varepsilon}$ \;

        $ \vec{\mu_i}^{(j)} \leftarrow \vec{\mu_i} + \vec{\delta\mu}^{(j)} $\;

        $ \vec{\delta\Sigma}^{(j)}  \leftarrow   (\vec{\mu}_i-\vec{\theta})(\vec{\mu}_i-\vec{\theta})^\top - (\vec{\mu_i}^{(j)}-\vec{\theta})(\vec{\mu_i}^{(j)}-\vec{\theta})^\top $  \;
    }

    Update $\vec{\mu_{i+1}} \leftarrow \vec{\mu_i} + \sum_j\vec{\delta\mu^{(j)}} / B$ \;

    Update $\vec{\Sigma_{i+1}} \leftarrow \vec{\Sigma_{i}} + \sum_j\vec{\delta\Sigma^{(j)}} / B$ \;
}
$q_{\bw}(\vec{\theta}) \leftarrow \mathcal{N}( \vec{\mu_{N}}, \vec{\Sigma_{N}})$ \;

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> sec_broader.tex <==
\section*{Broader Impact}

% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> sec_gsm_alt.tex <==
\section{Score-Matching Variational Inference}
\label{sec:gsm_alt}

We have a probabilistic model $\rmp(\theta, x)$ with latent variables $\theta$ and observations $x$. We want to calculate the posterior, \begin{align}
  \label{eq:posterior}
  \rmp(\theta \g x) = \frac{\rmp(\theta, x)}{\rmp(x)}.
\end{align}
But it is intractable, on account of its normalizing constant $\rmp(x)$.

To approximate it, we will use variational inference (VI). Generally, the goal of VI is to approximate an intractable posterior with a parameterized family of distrbutions $\rmq(\theta \s w)$. Typically, a VI method establishes a measure of closeness to the exact posterior and then optimizes the variational parameters to minimize it. Here we propose a new way to think about VI.

Suppose there are variational parameters $w^*$ that perfectly capture the posterior, i.e., where $\rmq(\theta \s w^*) = \rmp(\theta \g x)$ for all $\theta \in \Theta$.  This fact implies that \begin{align}
  \label{eq:score-match}
  \grad{\theta} \log \rmq(\theta \s w^*)
  =
  \grad{\theta} \log \rmp(\theta, x) \quad \forall \theta \in \Theta.
\end{align}
(The proof is in the appendix.) Notice the right side is an expression about the joint, not the posterior.

We will solve the VI problem by trying to find a $w$ that satisfies \Cref{eq:score-match}, a goal that reflects the principle behind \textit{score matching}~\cite{Hyvarinen:2005}. Score matching is a criterion for approximating a distribution that is known up to a normalizing constant. In \Cref{eq:posterior}, the data $x$ is fixed and the joint distribution $\rmp(\theta, x)$ is the unnormalized posterior. Thus finding variational parameters $w$ that satisfy \Cref{eq:score-match} is a score-matching approach to variational inference.

\parhead{Score-Matching VI.} With this goal in mind, \textit{score-matching VI} iteratively fits a variational family to be close to a posterior. At each iteration $t$, we sample a new value of $\theta_t$. We then minimally adjust the current variational approximation $w_t$ to a point that matches the scores at $\theta_t$.

In detail, each iteration samples $\theta$ and solves a constrained
optimization:
\begin{enumerate}[noitemsep]
\item Sample $\theta_t \sim \rmq(\theta \s w_{t-1})$.

\item Adjust the variational parameters:
  \begin{align}
    \label{eq:optimization}
    \begin{split}
      w_t
      =
      \arg & \min_w \kl{\rmq(\theta \s w_{t-1}) \, || \, \rmq(\theta \s w)} \\
      & \textrm{such that} \quad
      \grad{\theta}
      \log \rmq(\theta_t \s w) = \grad{\theta} \log \rmp(\theta_t, x).
    \end{split}
  \end{align}
\end{enumerate}
Intuitively this procedure produces a $\rmq(\theta \s w)$ that satisfies \Cref{eq:score-match} for all values of $\theta$.

\david{Can we say more? Where does this idea come from?  What is
  guaranteed?}

\parhead{Gaussian Score-Matching VI.} The utility of score-matching VI rests on the complexity of solving the constrained optimziation in \Cref{eq:optimization}. Suppose the variational family parameterizes a Gaussian, $w = \{\mu, \Sigma\}$. It might be a variational family with a full covariance, or a factorized (``mean field'') family, where $\Sigma$ is diagonal.

Then \Cref{eq:optimization} can be solved in closed form,
\begin{align}
  \mu_t
  &= \mu_{t-1}
    + A(w_{t-1}, \theta_t)
    (\grad{\theta} \log \rmq(\theta_t \s w_{t-1})
    - \grad{\theta} \log \rmp(\theta_t, x)) \\
  \Sigma_t
  &= (\mu_{t-1} - \theta_t) (\mu_{t-1} - \theta_t)^\top
    + (\mu_t - \theta_t) (\mu_t - \theta_t)^\top.
\end{align}
Intuitively, the algorithm adjusts the variational mean according to the degree that it violates the score-matching constraint. The function $A(w_{t-1}, \theta_t)$ is...

\david{Include the expression for $A()$ here, or defer to an appendix.}

With these closed form updates, Gaussian score-matching VI is a practical method for variational inference. It requires sampling from a Gaussian $\rmq(\theta \s w)$ and evaluating the gradient of the of the log joint $\grad{\theta} \log \rmp(\theta, x)$. (These are the same requirements as for black-box variational inference with reparameterization gradients.) The full algorithm is in \Cref{alg:gsm}.

\david{Include a demonstration here. Set an intractable model and show
  what happens (compared to BBVI) when we use SMVI. It makes things
  concrete for the reader.}

\david{Discuss properties, advantages, and limitations of the
  algorithm.}

\david{Clean up the algorithm.}

\begin{algorithm}[h]
\label{alg:gsm}
\input{gsm-alg.tex}
\caption{Gaussian Score-Matching VI}
\label{alg:gsm}
\end{algorithm}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

